ATP: AMRize Then Parse! Enhancing AMR Parsing with PseudoAMRs

As Abstract Meaning Representation (AMR) implicitly involves compound semantic annotations, we hypothesize auxiliary tasks which are semantically or formally related can better enhance AMR parsing. We find that 1) Semantic role labeling (SRL) and dependency parsing (DP), would bring more performance gain than other tasks e.g. MT and summarization in the text-to-AMR transition even with much less data. 2) To make a better fit for AMR, data from auxiliary tasks should be properly "AMRized" to PseudoAMR before training. Knowledge from shallow level parsing tasks can be better transferred to AMR Parsing with structure transform. 3) Intermediate-task learning is a better paradigm to introduce auxiliary tasks to AMR parsing, compared to multitask learning. From an empirical perspective, we propose a principled method to involve auxiliary tasks to boost AMR parsing. Extensive experiments show that our method achieves new state-of-the-art performance on different benchmarks especially in topology-related scores.

==> src/amrization.tex <==


Unlike conditional NLG tasks which can be directly applied to Seq2Seq training. Parsing Tasks involving structured target data should be first transformed to linear form before training. We name the process of transformation to mimic AMR's characteristics ``AMRization''.

The resources of shallow level annotations like Semantic Role Labeling and Dependency Parsing are richer and easier to annotate than that of AMR. Our  AMR parser would perform better if it could previously handle the shallow level tasks since the shallow level representations of sentence helps when conducting high level semantic analysis. To bridge the gap between shallow level annotations and AMR, we propose seven AMRization rules as follows. The rules can be divided into task-independent ones and task-dependent ones. The former serves as principles when starting to transform any possible tasks with structured data. The latter provides post transformation for specific task to further improve AMR parsing.

\subsection{Task Independent Rules}

\paragraph{Connected Directed Graph Formalization}
\label{sec:graph formalization} 
From formal perspective, the AMR is a connected directed acyclic graph. Our first principle when conducting AMRization is to transform the data structure of auxiliary task similar to that of AMR. For SRL, the original structure is forest consisting of multiple unconnected trees. By adding virtual root node and generating a directed edge from the virtual root to each root of SRL trees, the SRL annotations become a connected graph as depicted in Figure~\ref{fig:amrization}. For Dependency Parsing task, no extra procedure is needed since the structure of dependency tree already agrees with AMR in spite of reentrancy. For NLG task like Machine Translation, due to the lack of structure information, such transformation is not available.

\paragraph{Variable Restoration}
Following \citet{bevil-spring}, since AMR paring task uses graph-isomorphic linearization which requires special tokens <R0>,...,<Rn> to represent variables and handle coreference, we apply variable restoration by assign a numerical token to each node after the graph formalization.

\paragraph{Linearization}
After graph formalization and variable restoration, the graph structure should be linearized before doing seq2seq training. Following \citet{bevil-spring},we employ a DFS-based linearization with special tokens to indicate variables and parentheses to mark visit depth, which is the best linearization method according to \citet{bevil-spring}.

\subsection{Transform SRL to Pseudo AMR} AMR captures the predicate-argument structure of one sentence which is also the main task of Semantic Role Labeling. Actually, SRL is an important sub-task of AMR parsing \citep{ban-AMR,dam-smatch-incremental}. As shown in Figure \ref{fig:srl_dp_amr}, the SRL and AMR of sentence "The boy wants to leave" carry much resemblance. 1) They both locate the predicates (want, leave) of sentence and conduct word-sense disambiguation according to PropBank. 2) They both capture the multiple arguments of center predicate. 
% 浅层任务可以帮助AMR Parsing

However, it is undeniable that there are gaps in both formal and semantic level between SRL and AMR. From formal perspective: 1) AMR is a connected directed graph while the sturcture of SRL is forest. This can be handled through \textbf{Graph Formation} as discussed in Section~\ref{sec:graph formalization}. 2) Reentrancy is an important and nontrivial feature of AMR. Though SRL capture similar predicate-argument structure to AMR, there is no reentrancy. From semantic level, the arguments of SRL are token spans (eg. the boy, that boy, this boy) while the argument of AMR is concept (boy). The latter is more abstract and capture deeper semantics. In following sections, we propose \textbf{Argument Reduction} and \textbf{Reentrancy Restoration} as depicted in Figure\ref{fig:amrization}, attempting to bridge the formal and semantic gap between SRL and AMR.
% 任务形式存在较大差异，但可以人为修改，更像amr 1.形式层面 2.语义层面。

\paragraph{Argument Reduction}We use dependency parser from Stanford CoreNLP Toolkit \cite{corenlp} to do the argument reduction. We run dependency parsing if the argument of current predicate is more than one token and replace the original token span with the root token in the dependency structure. Similar method has been to applied by \cite{zhang-etal-2021-comparing} to find the head of token spans of argument.

\paragraph{Reentrancy Restoration} We design an heuristic algorithm based on DFS to restore reentrancy in SRL, transforming the tree structure to graph. The core idea of the restoration is that we create a variable when the algorithm first sees a node. Next time if meeting node with the same name, the destination of the edge will be referenced to the variable we have created at first. The pseudo code is in Appendix~\ref{alg:reen}


\subsection{Transform Dependency Structure to Pseudo AMR} Similar to AMR parsing, dependency parsing (DP) builds a directed tree structure from tokens of a sentence. DP can be viewed as an edge prediction task since all nodes in the graph are given while AMR Parsing requires predicting both nodes and edges, which makes DP a sub-task of AMR parsing from the perspective of edge prediction. There are three main methods to do dependency parsing: Transition-based \citep{Chen2014AFA}, Graph-based \citep{Kiperwasser2016SimpleAA}, Seq2Seq-based \citep{Li2018Seq2seqDP}, which are the same as AMR parsing suggesting the resemblance between AMR Parsing and Dependency Parsing. Different from constituency parsing (CP), there is no none-terminal in both AMR and DP, which makes DP more similar to AMR than CP.

Formal and semantic gap also exist between DP and AMR. First, some relations in dependency parsing focuses on shallow syntax like (punctuation, delimiters) which are far from high-level semantic relations in AMR. Second, similar to SRL, the basic node of dependency structure is token while that of AMR is concept, which capture deeper syntax-independent semantics . We use \textbf{Redundant Relation Removal} and \textbf{Token Lemmatization} to better transform DP to Pseudo AMR.

\paragraph{Redundant Relation Removal} We remove some of the dependency relations that are far from relations in AMR eg. :ROOT, :DET. However, the choice of best redundant relations is an NP-hard problem. We reserve the full exploration of relation removal for further studies. By removing some relations of the dependence, the parsing result become more sparse compared with original DP tree, forcing the model to ignore some semantics-unrelated tokens during seq2seq training.


\paragraph{Token Lemmatization} 
We use NLTK \citep{bird-2006-nltk} to conduct token lemmatization on the node of dependency tree. Together with the smart-initialization \citep{bevil-spring} by setting the concept token's embedding as the average of the subword constituents, the vector of lemmatized token (want) becomes closer to the vector concept (want-01) in the embedding matrix, therefore requiring the model to capture deeper semantic when conducting DP task.




==> src/dataset.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/amri.pdf}
    \caption{AMRization methods for SRL and DP}
    \label{fig:amrization}
\end{figure*}

\subsection{Auxiliary Task Selection}

we choose from a wide range of tasks including summarization\citep{Hermann2015TeachingMT,chen-etal-2021-dialogsum}, translation and parsing\citep{ptb3,Weischedel2017OntoNotesA} to evaluate the contribution of different auxiliary task for AMR parsing. We use gold annotation data in all tasks and maintain a close number (\textasciitilde40k) of examples for each task for fair comparison. Due to space limitation, we list the full dataset description in Appendix~\ref{app:dataset_des}. 

% \subsection{Summarization}

% \paragraph{\textsc{CNN/DM}\citep{Hermann2015TeachingMT}}The CNN / DailyMail Dataset is an English-language dataset containing news articles as written by journalists at CNN and the Daily Mail. The dataset is widely accepted as benchmark to test models' performance of summarizing . We select 40k training data for fair comparison. 
% \paragraph{\textsc{DialogSum}\citep{chen-etal-2021-dialogsum}}
% The Real-Life Scenario Dialogue Summarization (\textsc{DialogSum}), is a large-scale summarization dataset for dialogues. Unlike \textsc{CNN/DM} which focuses on monologue news summarization, \textsc{DialogSum} covers a wide range of daily-life topics in the form of spoken dialogue. We use all the training data (13k) to conduct the intermediate training.

% \subsection{Translation}

% \paragraph{\textsc{WMT14 EN-DE}} We select 40k training examples from WMT14 EN-DE training set to form EN-DE and DE-EN translation intermediate task.

% \subsection{Dependency Parsing}

% \paragraph{\textsc{Penn Treebank}\citep{ptb3}} The Penn Treebank (PTB) project selected 2,499 stories from a three year Wall Street Journal (WSJ) collection of 98,732 stories for syntactic annotation. We only utilize the dependency structure annotations to form our intermediate dependency parsing task. There are 39k sentences for dependency parsing. 

% \subsection{Semantic Role Labeling}
% \paragraph{\textsc{OntoNotes}\citep{Weischedel2017OntoNotesA}} The OntoNotes project is built on two resources, following the \textsc{Penn Treebank}\citep{ptb3} for syntax and the \textsc{Penn PropBank} for predicate-argument structure. We select 40k sentences with SRL annotations to form intermediate task.



% \include{AMRization/table/dataset}

==> src/task.tex <==
Following previous methods \cite{bevil-spring, xu-seqpretrain, ge-seq2seqamr}, we formulate AMR parsing as a sequence-to-sequence generation problem.
Formally, given a sentence $\mathbf{x} = (x_1, x_2, ..., x_N)$, the model needs to generate a linearized AMR graph $\mathbf{y}=(y_1, y_2, ..., y_M)$.
As shown in Figure \cite{xx},
following \cite{bevil-spring}, the AMR graph was linearized with Depth-First Search (DFS) traversal, and variables in AMR are set to a a series of special tokens \textit{<R0>, <R1>, ..., <Rk>}.



==> table/ablation.tex <==
\begin{table}[t]
\centering
\scalebox{0.92}{
\begin{tabular}{lcc} \toprule
Model & \textsc{AMR2.0} & \textsc{AMR3.0} \\
\midrule
Ours  &                    84.6 $\pm$0.1  &    84.1 $\pm$0.1     \\
w/o structure curriculum   & 84.2 $\pm$0.2   &    83.4 $\pm$0.1     \\
w/o instance curriculum &  84.3 $\pm$0.1   &    83.7 $\pm$0.2    \\ 
w/ \ \ inverse curriculum  &  83.7 $\pm$0.2   &    82.8 $\pm$0.1 \\     
\bottomrule  
\end{tabular}}
\caption{The effect of our proposed curriculums on AMR2.0 and AMR3.0. We report the \textsc{smatch} scores with standard deviation on $3$ different seeds. `w/ inverse curriculum' trains the model from deep to shallow sub-AMR graphs, and hard to easy instances.}
\label{tab:abla-study}
\end{table}

==> table/dataset.tex <==
\begin{table}[h]
\centering
\scalebox{0.95}{
\begin{tabular}{ccccc}
        \toprule
         Dataset &Task & Train & Validation \\
        \midrule
        CNNDM & Summarization & 40k & 1k \\
        DialogSum & Summarization & 13k & 0.5k \\
        EN-DE & Translation & 40k & 3k \\
        DE-EN & Translation & 40k & 3k \\
        Ontonotes & SRL & 40k & 1.5k \\
        PTB3 & DP & 39k & 1.7k \\

        \bottomrule
    \end{tabular}}
    \caption{Dataset introduction}

    \label{tab:dataset}
\end{table}

==> table/dp_amrizatiton.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{1\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
        \toprule
                ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
                \multirow{2}{*}{NoWSD} &
                \multicolumn{4}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
                \cmidrule(r){6-9} \cmidrule(r){10-12} 
        ~ & ~ & ~ & ~& ~ & Conc. & NER & Neg. & Wiki. & Unll. & Reen. & SRL \\
        \midrule
        

        \multirow{7}{*}{\rotatebox[origin=c]{90}{{2.0}}}      
                                          
        ~& \citet{bevil-spring}       &N     & 83.8  & 84.4 & 90.2 & 90.6 & 74.4 & 84.3 & 86.1 & 70.8 & 79.6 \\
        ~& \citet{bevil-spring} (w/ silver)   &200k     & 84.3 & 84.8 & 90.8 & 90.5 & 73.6 & 83.1 &  86.7 &  72.4 & 80.5 \\
        ~& \textbf{Ours (w/ Dependency Parsing) } \\
        ~& - w/ Trivial Linearization &39k  \\
        ~& - w/ Redundant Relation Removal (RRR) &39k &     \\
        ~& - w/ Lemmalization (Lemma)  &39k & 84.7 	& 	85.2 	&90.2 	&91.2 	&75.0 	&83.8 	&88.0 &74.1 	&83.0   \\
        ~& - w/ RRR + Lemma  &39k  & \textbf{85.0}            & \textbf{85.4} & \textbf{90.4} & \textbf{92.5}  & \textbf{74.7} &  84.1  &  \textbf{88.2}  &  \textbf{74.7} & \textbf{83.1} \\
        \bottomrule
    \end{tabular}
    }\caption{Analysis on DP's AMRization methods}

    \label{tab:srl_amr}
\end{table*}



==> table/task_select.tex <==


\begin{table*}[htb]
    \centering
    \resizebox{1\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
        \toprule
                ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
                \multirow{2}{*}{NoWSD} &
                \multicolumn{4}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
                \cmidrule(r){6-9} \cmidrule(r){10-12} 
        ~ & ~ & ~ & ~& ~ & Conc. & NER & Neg. & Wiki. & Unll. & Reen. & SRL \\
        \midrule
        

        \multirow{7}{*}{\rotatebox[origin=c]{90}{{2.0}}}      
                                          
        ~& \citet{bevil-spring}       &N     & 83.8  & 84.4 & 90.2 & 90.6 & 74.4 & \textbf{84.3} & 86.1 & 70.8 & 79.6 \\
        ~& \citet{bevil-spring} (w/ silver)   &200k     & 84.3 & 84.8 & \textbf{90.8} & 90.5 & 73.6 & 83.1 &  86.7 &  72.4 & 80.5 \\
        ~& \textbf{Ours (w/ NLG Task) } \\
        ~& - w/ DialogSum & 13k & 84.5 &84.9 & 90.2&91.5 &74.8 &82.0 &87.8 &74.1 & 82.7 \\
        ~& - w/ CNNDM   & 40k & 84.4 &84.9 & 90.1& 91.5&74.8 &82.7 &87.7 & 74.6& 82.8 \\
        ~& - w/ DE-EN   & 40k &84.4 &84.9 &89.9&90.8&73.3&83.1&87.6&74.1&82.8\\ 
        ~& - w/ EN-DE   & 40k &84.0 &84.3 &89.7 &90.9 &74.3 &83.2 &87.1 &73.5 &81.9\\ 
        ~& \textbf{Ours (w/ Parsing Task) } \\
        ~& - w/ DP & 39k & 85.0          & 85.4 & 90.4 & \textbf{92.5}  & 74.7 &  84.1  &  \textbf{88.2}  &  74.7 & 83.1 \\    
        ~& - w/ SRL &   40k  &\textbf{85.1}   &\textbf{85.6}  &90.4  & 91.4  & \textbf{75.7} &  83.6 & \textbf{88.2} & \textbf{75.0}  &  \textbf{83.5}       \\    
        \bottomrule
    \end{tabular}
    }
    \caption{Analysis on Task Selection}

    \label{tab:task_sel}
\end{table*}
